Towards Superior Quantization Accuracy: A Layer-sensitive Approach

Large Vision and Language Models have exhibited remarkable human-like intelligence in tasks such as natural language comprehension, problem-solving, logical reasoning, and knowledge retrieval. However, training and serving these models require substantial computational resources, posing a significant barrier to their widespread application and further research. To mitigate this challenge, various model compression techniques have been developed to reduce computational requirements. Nevertheless, existing methods often employ uniform quantization configurations, failing to account for the varying difficulties across different layers in quantizing large neural network models. This paper tackles this issue by leveraging layer-sensitivity features, such as activation sensitivity and weight distribution Kurtosis, to identify layers that are challenging to quantize accurately and allocate additional memory budget. The proposed methods, named SensiBoost and KurtBoost, respectively, demonstrate notable improvement in quantization accuracy, achieving up to 9% lower perplexity with only a 2% increase in memory budget on LLama models compared to the baseline.

==> Makefile <==
all:    paper

paper: paper.tex
	pdflatex -sync-tex=1 -shell-escape paper
	bibtex paper
	pdflatex -sync-tex=1 -shell-escape paper
	pdflatex -sync-tex=1 -shell-escape paper

clean:
	rm -f *.aux *.log *.xml *.out paper.pdf *.bcf *.toc *.blg *.bbl *.dvi *.fls *.tgz
	rm -fr _minted-paper/ tmp/

arxiv:
	tar -czvf preprint.tgz \
		Makefile \
		PRIMEarxiv.sty \
		paper.tex \
		paper.bbl \
		figs/Llama-2-7b-outlier-1_self_attn_o_proj.jpg \
		figs/Llama-2-7b-outlier-31_self_attn_o_proj.jpg \
		figs/circos-Llama-3-8B-4.25.pdf \
		figs/circos-sb22-Llama-3-8B-4.25.pdf \
		figs/lpnorm-07.pdf \
		figs/lpnorm-squred.pdf \
		figs/ppl-decr-mem-inc.pdf \
		figs/ppl-kbab-Llama-2-13B-WikiText2.pdf \
		figs/ppl-kbab-Llama-3-8B-WikiText2.pdf \
		figs/ppl-sbab-Llama-2-13B-WikiText2.pdf \
		figs/ppl-sbab-Llama-3-8B-WikiText2.pdf \
		figs/ppl-sk-Llama-2-13B-WikiText2.pdf \
		figs/sensi-ft-llama.pdf \
		figs/sensi-llama-bit-budget.pdf \
		figs/sensi-qnt-mtd.pdf \
		figs/wtl-llama-comparison.pdf \
		algo-outlier-detection.tex \
		figure-llama2-7b-outliers-3d.tex \
		figure-quant-cfg-allot.tex \
		figure-sensi-ds-meth.tex \
		figure-wtl-llama.tex \
		figure-sk-wikitext.tex \
		figure-quant-cfg-sb22.tex \
		figure-ppl-decr-extra-mem.tex \
		figure-sensi-llama.tex \
		figure-sensi-ft-llama.tex \
		table-hqq-bit-budget.tex \
		table-method-eval-matrix.tex \
		appendix.tex


==> figure-quant-cfg-allot.tex <==
%!TeX root = report.tex

\begin{figure*}[t]
  \centering
\includegraphics[width=0.95\textwidth]{circos-Llama-3-8B-4.25.pdf}
\caption[Quantization Config Allocation Comparison]{
This figure presents a comparison of quantization configuration allocations as
determined by SensiBoost, KurtBoost, HQQ and MXQ for the Llama-3-8B model,
under a bit budget of 4.25. The colored rings represent the assigned
quantization configurations denoted as b2g128 through b8g32, while the text in
the center indicates the perplexity scores. As demonstrated by this figure, MXQ
allocates far more configurations than other approaches, however, the
perplexity scores are considerably worse than others. For optimal clarity, the
figure is best viewed in color and with zoom.
}
\label{fig:llama-8b-cfg-allocation}
\end{figure*}

